RCAgent: Cloud Root Cause Analysis by Autonomous Agents with Tool-Augmented Large Language Models

Large language model (LLM) applications in cloud root cause analysis (RCA) have been actively explored recently. However, current methods are still reliant on manual workflow settings and do not unleash LLMs' decision-making and environment interaction capabilities. We present RCAgent, a tool-augmented LLM autonomous agent framework for practical and privacy-aware industrial RCA usage. Running on an internally deployed model rather than GPT families, RCAgent is capable of free-form data collection and comprehensive analysis with tools. Our framework combines a variety of enhancements, including a unique Self-Consistency for action trajectories, and a suite of methods for context management, stabilization, and importing domain knowledge. Our experiments show RCAgent's evident and consistent superiority over ReAct across all aspects of RCA -- predicting root causes, solutions, evidence, and responsibilities -- and tasks covered or uncovered by current rules, as validated by both automated metrics and human evaluations. Furthermore, RCAgent has already been integrated into the diagnosis and issue discovery workflow of the Real-time Compute Platform for Apache Flink of Alibaba Cloud.

==> table/embedding.tex <==
% root cause作为主表，基础的自动评价表现，会附上模型评测，作为基础评价手段. pass rate删掉

\begin{table}[tbp!]

\small

\caption{
    \label{tab:embedding}
    Performance of RCAgent with different embedding models. 
    % The metric is calculated between the predicted root cause and solution, and annotated root causes due to lack of solution annotation. 
    % MTEB scores for 
    The OpenAI model is presented for reference. 
}
\vspace{-3mm}
\resizebox{\linewidth}{!}{
\begin{tabular}{l | c | c c  }
\toprule
\multicolumn{1}{l|}{Model} 
 & MTEB  & BLEURT & BARTScore \\ 
\midrule

GTE-LARGE
& 63.13 & 36.74 & -5.43 \\ 
\textit{Text-Embedding-Ada-002}
& 60.99 & - & - \\
MPNet
& 57.78 & 37.48 & -5.44 \\ 
ST5-BASE
& 55.27 & 36.08 & -5.51 \\ 
MiniLM-L12-multilingual
& 52.44 & 35.30 & -5.65 \\ 
% SimCSE-Bert-sup
% & 48.72 & 11.70 & 30.14 \\ 
% simcse感觉是跑得有问题，加载了一个不正确的模型

\bottomrule

\end{tabular}

}
\vspace{-3mm}
\end{table}
